High frequency study of FRB 20180916B using the 100-m Effelsberg radio telescope

FRB 20180916B is a repeating fast radio burst (FRB) with an activity period of 16.33 days. In previous observations ranging from $\sim 150-1400$ MHz, the activity window was found to be frequency dependent, with lower frequency bursts occurring later. In this work, we present the highest-frequency detections of bursts from this FRB, using the 100-m Effelsberg Radio Telescope at 4$-$8 GHz. We present the results from two observing campaigns. We performed the first campaign over an entire activity period which resulted in no detections. The second campaign was in an active window at 4$-$8 GHz which we predicted from our modelling of chromaticity, resulting in eight burst detections. The bursts were detected in a window of 1.35 days, 3.6 days preceding the activity peak seen by CHIME, suggesting the chromaticity extends to higher frequency. The detected bursts have narrower temporal widths and larger spectral widths compared to lower frequencies. All of them have flat polarization position angle sweeps and high polarization fractions. The bursts also exhibit diffractive scintillation due to the Milky Way, following a $f^{3.90\pm0.05}$ scaling, and vary significantly over time. We find that burst rate across frequency scales as $f^{-2.6\pm0.2}$. Lastly, we examine implications of the frequency dependency on the source models.

==> makefile <==
SHELL:=/bin/bash
all:main.tex
	latexmk -pdf -silent 

debug:main.tex
	latex $< ;\
	open main.pdf &

old:main.tex
	latex $< ;\
	bibtex rm ;\
	latex $< ;\
	latex $< ;\
	pdflatex $< ;\
	open main.pdf &

.PHONY: gadd
gadd:
	@read -p "git commit description: " DESCRIPTION;\
	git add . ;\
	git commit -m "$$DESCRIPTION" 

.PHONY: gpush
gpush:
	git push origin;

gpull:
	@read -p "remote name:" REMOTE;\
	git pull $$REMOTE master --allow-unrelated-histories

gcheck:
	git log -p -2

gremote:
	git remote add overleaf $$URLoverleaf
	git remote add github $$URLgithub

.PHONY: clean
clean: 
	rm -f *.dvi  *.aux *.blg *.toc *.out *.fdb_latexmk *.log *.synctex.gz *.fls

